Resource-Aware Heterogeneous Federated Learning using Neural Architecture Search

Federated Learning (FL) is extensively used to train AI/ML models in distributed and privacy-preserving settings. Participant edge devices in FL systems typically contain non-independent and identically distributed (Non-IID) private data and unevenly distributed computational resources. Preserving user data privacy while optimizing AI/ML models in a heterogeneous federated network requires us to address data and system/resource heterogeneity. To address these challenges, we propose Resource-aware Federated Learning (RaFL). RaFL allocates resource-aware specialized models to edge devices using Neural Architecture Search (NAS) and allows heterogeneous model architecture deployment by knowledge extraction and fusion. Combining NAS and FL enables on-demand customized model deployment for resource-diverse edge devices. Furthermore, we propose a multi-model architecture fusion scheme allowing the aggregation of the distributed learning results. Results demonstrate RaFL's superior resource efficiency compared to SoTA.

==> cvpr2023/07_supplementary_materials.tex <==
\newpage
\onecolumn
\section{\centering{Supplementary experimental results}}

\label{sec:appendix}


\subsection{Summary}
In supplementary materials, we explore the cases where \proj fails to outperform baselines. This is quite expected as every design has its own strengths and weakness. There is no singular solution that universally addresses all possible FL settings.
We summarized scenarios where \proj shows in advanced: 
1. bandwidth matters.
2. public data available  
3. edge devices are resource limited.
4. large scale.


\subsection{Experiments}
We conducted extensive experiments to evaluate \proj and summarized our experiments into five sections: learning efficiency, communication efficiency, system heterogeneity, resource utilization, and ablation study.
In learning efficiency, we analyze the optimization ability for training the target model. The communication efficiency experiment investigates the communication cost incurred by client-server updates. 
In our system heterogeneity experiment, we highlight the advantage of \proj across systems with varying resources. %in different system hetero settings.
In the utilization experiment, we measure the overall resource use efficiency. Lastly, we conduct a comprehensive ablation study.

\subsection{Experimental Setup}
% \noindent\textbf{Datasets and models.} We conduct experiments on datasets inline with baselines: CIFAR-10/100~\cite{krizhevsky2009cifar}, FEMNIST~\cite{caldas2019leaf} and Tiny ImageNet~\cite{russakovsky2015imagenet} under Non-IID benchmark settings~\cite{li2022niidbench}. 
% We deploy resource-aware deep learning models sampled from MobileNetV2/V3~\cite{howard18mobilenetv2,howard19mobilenetv3} or ResNet \cite{he2016resnet} super-network in different cases. 
% Two popular datasets in the field: Cifar-10/100~\cite{krizhevsky2009cifar} and FEMNIST~\cite{caldas2019leaf} are used for training on local client. 
% In the non-IID setting, each client is assigned a sample proportion of each label based on the Dirichlet distribution (with concentration $\alpha$). Specifically, we sample $p_k \sim Dir_N(\alpha)$ and assign a $p_{k,j}$ proportion of the instances to client $j$. Here we choose the $\alpha = 0.1$. 
% In contrast, in baselines, we deploy a uniformed architecture sampled from MobileNetV2/V3 and ResNet correspondingly.
To avoid confusion, we identify networks by their capacity~(via FLOPs), eg. we identify ResNet-34 as: ResNet with $76$ MFLOPs.
% Additionally, our experiments also involve traditionally over-parameterized models, such as VGG-11/16~\cite{simonyan2015vgg}, for highlight comparison.
\\
\textbf{FL and Non-IID settings.} All our experiments are conducted on benchmark Non-IID settings~\cite{li2022niidbench}. 
Specifically, we use label heterogeneity to set up Non-IID.
We consider the following three scenarios: (a) traditional FL setting, (b) public data with ensemble knowledge distillation, and (c) transfer learning with NAS. 
With CIFAR-10/100, we experiment on different number of clients from $30$ to $100$ and sample $10\%$ to $70\%$ clients for communication, while with FEMNIST, we experiment on $3000$ clients.  \\
\textbf{Public data settings.} We tried different public data to perform ensemble distillation, including 10k randomly unlabled data points sampled from Tiny ImageNet, 10k randomly unlabled data points sampled from CINIC-10 (after removing overlaping with cifar-10), and 5k data points split from CIFAR-10 training data.
\\
\textbf{NAS settings.} We conduct neural architecture search on pre-trained OFA~\cite{cai20ofa} super-networks on ImageNet~\cite{russakovsky2015imagenet}. Super-network architectures involved in the experiments include ResNet, MobileNetV2, and MobileNetV3. Resource-aware models will be sampled from the super-networks. According to the FL settings, pre-trained weights inherited from super-network can be reset or transferred accordingly.
% the resource constraints, different sub-network will be selected from those super-network to each local devices. 
Detailed information is specified in the subsections. \\
\textbf{Knowledge Network setting.} We sampled a tiny network (in terms of FLOPs) from super-network as the knowledge network. 
In \proj, the network capacity we shows are the integrated capacity of knowledge network and specialized local network. For instance, we deploy a 30 MFLOPs ResNet and a 10 MFLOPs knowledge network at local, we use 40 MFLOPs (30 MFLOPs + 10 MFLOPs) to identify the network capacity we deployed at edge in \proj.

% Commonly, there is a trade off between FL performance and knowledge network size. However, in ablation study~(section \ref{sec:ablation}) we show small knowledge network is an efficient choice. 



%All the baselines are implemented following the non-IID benchmark federated learning setting \cite{li2022niidbench}.



%and FedDF \cite{lin20ensemble} (for model fusion). 




% \input{content/figtex/f_train_effi.tex}


\subsection{Learning Efficiency}
\label{sec:apendix:le}
% \input{cvpr2023/figtex/learning_efficiency/converge_accuracy.tex}

\input{cvpr2023/Figures/f_avg_100_01_cifar100.tex}
% \input{cvpr2023/Tables/apdx/t_learning_efficient_cifar100.tex}

% \input{cvpr2023/Tables/t_learning_efficiency.tex}
Due to the page limits, in manuscripts, we mainly show the results on CIFAR-100. In this section we provides supplementary results on learning efficiency evaluation, including results on CIFAR-10 and various FL settings.
As shown in Figure~\ref{fig:converge_acc}, we conducted experiments on comprehensive FL settings, from 30 clients to 100 clients and different participating rate. \proj shows stable results and consistently outperform baselines.
Intuitively, Figure~\ref{fig:learn_efficiency} shows training supplementary training logs of \proj.
\proj achieves a higher convergence accuracy while requiring fewer rounds to achieve the target precision compared to baselines. For instance, in the 30 clients FL setting, it ahieves at $70\%$ final accuracy, which is $10\%$ higher than other 3 baselines~(Figure~\ref{fig:learn_efficiency} (II)(1), (II)(3), (II)(4)). There are some exceptions where \proj does not outperform the baselines in case of 100 clients with $40\%$ sample rate (Figure~\ref{fig:learn_efficiency} (II)(3)). \proj with smaller sub-network achieved a converged accuracy of $55\%$, slightly lower than $57\%$ by FedAvg and FedNova. However, it is worth noting that \proj uses far less bandwidth per communication rounds~($1.6$ GB versus $2.8 $GB and $5.6$ GB for FedAvg and FedNova respectively) compared to the baselines. Thus with a small sacrifice in accuracy, we make a larger gain in terms of communication cost.  Compared to the local dataset~(CIFAR10/100), it improves the performance of both the global and local models. 

% It is worth mentioning that \proj shows superior in resource-friendly. We conducted 2 sets of experiments on ResNets in Figure~\ref{fig:vanilla}, where we set RaFL to deploy a similar and far less network capacity compare to baselines. In both settings, RaFL outperform baselines, that is because \proj take the advantage of NAS, deploying high-performance neural architecture to edge clients, huge amount of redundant neural parameter been pruned before training, and hence, less computational resource are needed to achieve target model performance.


% RaFL equipped with ensemble distillation improved the performance with vanilla aggregation only.   
% \proj achieves a higher convergence accuracy while requiring fewer rounds to achieve the target precision compared to baselines. For instance, in the 30 clients FL setting, it ahieves at $70\%$ final accuracy, which is $10\%$ higher than other 3 baselines~(Figure~\ref{fig:learn_efficiency} (II)(1), (II)(3), (II)(4)). There are some exceptions where \proj does not outperform the baselines in case of 100 clients with $40\%$ sample rate (Figure~\ref{fig:learn_efficiency} (II)(3)). \proj with smaller sub-network achieved a converged accuracy of $55\%$, slightly lower than $57\%$ by FedAvg and FedNova. However, it is worth noting that \proj uses far less bandwidth per communication rounds~($1.6$ GB versus $2.8 $GB and $5.6$ GB for FedAvg and FedNova respectively) compared to the baselines. Thus with a small sacrifice in accuracy, we make a larger gain in terms of communication cost.  Despite the dissimilarity of the public data~(Sampled 10k data points from TinyImagenet in this case) compared to the local dataset~(CIFAR10/100), it improves the performance of both the global and local models. 

% \textbf{Explanation of baselines SCAFFOLD.} We follow the Non-IID benchmark implementation, we found that the gradient exploded

\subsection{Communication Efficiency}
Table~\ref{tab:target_acc} shows the detailed information refers in Figure~\ref{fig:comm_target}. Communicating smaller knowledge network and need fewer rounds to achieve target accuracy help \proj build communication efficient federated leanring.






% % \subsection{Inference acceleration}



% \input{cvpr2023/Tables/t_converged_acc}

\input{cvpr2023/Tables/t_target_acc}


% \subsection{Resource-aware System Heterogeneity}
% \label{sec:append_resource_hete}
% \input{cvpr2023/Tables/t_resource_aware_append.tex}
% % \input{cvpr2023/Figures/f_resource_aware}

% % \input{cvpr2023/Figures/f_client_overhead}
% %\proj, with its resource-aware NAS, demonstrates superiority under various resource heterogeneity.
% We conduct an ablation experiment to investigate \proj's ability to deal with resource heterogeneous settings. 
% Concretely, as shown in Figure~\ref{fig:client_overhead}, in a FL resource heterogeneous setting, we give every single client a resource overhead specified by MFLOPs, the model deployed on the clients should within the limit of given resource overhead. 
% % Since the xx is happens in edge device, here we consider traditional FL. In ablation study, we other xx has the same trend.
% As shown in Figure~\ref{fig:resource_aware}, \proj exhibits a stable optimizing ability under different system heterogeneity. Under extreme highlight settings, the average $48.01$ MFLOPs overhead compare to $79.70$ MFLOPs, where the training process shows they have similar learning trend and final accuracy despite having nearly $2\times$ difference in resource constraints. 
% Furthermore, 
% Figure~\ref{fig:client_overhead} shows edge clients' performance, 
% % The shade of color represents corresponding computational power. 
% edge clients show similar performance despite the variance in their network capacities. This can be attributed to the optimal architecture query performed by NAS under the provided resource constraints.

% Furthermore, \proj shows significant resource utilization efficiency. As in Table Table~\ref{tab:resource_aware}, at least $90\%$ resource  were utilized by \proj across different constraints and model architectures with the highest being $99\%$. In contrast to single model deployment in baselines, their resource utilization would be limited by the lowest resource capacity clients.
% For instance, as resource heterogeneous in Figure~\ref{fig:client_overhead}, even though some clients can accommodate up to XX MFLOPs, due to the single model deployments, the model capacity have to satisfy the lowest resource constraint, which is XX MFLOPs. Hence, leading to a XX\% poor resource utilization.
% % if the resource limit is $79.70$ MFLOPs for ResNet, we can only deploy the model with $76$ MFLOPs, not the one with $152$ MLFOPs. If the resource limit is $20$ MFLOPs for MobileNet, we can only use $xx$ MFLOPs model.

% In both cases, the their accuracies are much lower than \proj (as recorded in Table~\ref{tab:converged_acc}). In other words, our method can be personalized well for each clients with different capability limitation, which is a typical scenario in practical Federated Learning.


% % Hence their resource use efficiency is only $75\%$ on $79.70$ MFLOPs constraints. \proj achieves $13.3\%$ more resource utilization under similar settings.

% % table (comprehensive table shows in supplementary material, table xx), here we only compare with fedNova, since it performs better in baselines:
% % xxx xx

% % a table, a figure(training details).
% % conclusion: although xx some converge slower, but xx.

% % \subsubsection{resource utilization}

% %
\subsection{Extra burdens of Knowledge Networks}
\label{sec:apdx_extra_kn_cost}
When we initially evaluate \proj, we concerned that adding knowledge network and perform local deep mutual learning might add extra computational burdens at edge.
Hence, we build two FL environments and designed the following experiments:
In the first FL environment, we deployed a 12 MFLOPs MobileNet-V3 and a 8 MFLOPs MobileNet-v3 knowledge network at every single local client.
In the second FL environment, we deployed a 20 MFLOPs MobileNet-V3, at every single local client, and directly local update the model with SGD algorithm without the knowledge distillation.
To make a relatively fair comparison, and avoid any lottery results, we train the above two FL environments 500 rounds separately in the same nodes and the same type of GPU (NVIDIA v100s). Since our experimental platform is an HPC server, other jobs running on the HPC ontology might affect the actual training time, and a few deviations may present, but it is acceptable. 
We surprisingly found that the second FL setting takes 49 hours and 19 minutes, while the first FL setting takes 48 hours and 25 minutes to finish training, even faster than only optimizing a single model.
We further consult an expertise researcher in related areas, the reason is: when we perform deep mutual learning on the local model (12 MFOLOPs network) and knowledge network (8 MFLOPs network), our python deep learning framework will create a corresponding computational graph for each network and load in memory, and use them for gradient calculation. We can view the two computational graphs as disconnected computational graphs. Hence, training a disconnected computational graph (with a 12 MFLOPs sub-graph and 8 MFLOPs sub-graph) takes a similar computational cost as we train a single 20 MFLOPs computational graph.
\input{cvpr2023/Tables/t_kd.tex}


\subsection{Comparison with KD-based FL}
\label{sec:apdx_kdbaselines}
In our experiment, as Table~\ref{tab:kd_baselines} shows, we found that using knowledge distillation to aggregate local models may not improve the FL's learning efficiency. The performance of knowledge distillation highly depends on the similarity of public data and local data. Pure knowledge distillation does not apply to all general FL environments.
In this section, we compare \proj with knowledge distillation baseline FedDF~\cite{lin2020feddf} under different public data.
FedDF aggregates local models by ensemble local models and distillates the ensemble knowledge to the global model. \proj is more robust, in each round of communication, \proj first initializes the global knowledge network by weighted averaging local knowledge networks via Equation~\ref{eq:aggre}, and then optionally performs ensemble knowledge distillation. In case the public data drifts significantly from the overall local data distribution in FL, \proj can suffer less negative effects.
% However, ensemble knowledge distillation doesn’t always
% improve performance. It’s dependent on the similarity of
% the public and private client data distributions


\subsection{Analysis \proj and other FL NAS method}
\label{sec:apdx_nas}
In this section, we analyze the pros and cons of mainstream NAS methods in FL with RaFL, such as FedNAS~\cite{he2020fednas} and DecNAS~\cite{xu2020decnas}.
Firstly, we have different objections. Both FedNAS~\cite{he2020fednas} and DecNAS~\cite{xu2020decnas} target to optimize the NAS super-network via federated learning on user private data. FedNAS deploy NAS super-networks to every local client and perform NAS before local updating. Then each client updates a sub-network derived from the local NAS super-network and aggregate local sub-networks to the corresponding part of the super-network in the cloud. Similarly, DecNAS aims to optimize NAS super-network in a decentralized manner and utilize data and computational resources at the edge. 

Both of the methods may not get efficient neural architecture. For instance, in NAS, the search process usually starts after the super-network is well-trained, and it requires us to maintain a look-up table to track high-performance architectures under certain resource constraints.
However, FedNAS perform a neural architecture search at the very beginning of the training, and it may not get high-performance architectures.
Second, existing methods may not efficiently address resource heterogeneity at the edge. existing methods only consider the inference when in applications, and they directly deployed supernet at the edge. For example, FedNAS directly perform neural architecture at the edge. Neural architecture search is computationally costly, which may not fit resource constraints edge devices. 
Lastly, optimizing super-networks in FL environments are easily leading to divergence. It may work when the number of clients is limited. Nevertheless, when the FL becomes large-scale, for instance, 100 clients on CIFAR-100 in our experiments, where each client only allocated 500 data points, it's almost impossible to converge the over-parameterized super-networks. In our experiments, we show that our baselines suffer remarkably over fittings.  

In RaFL, we ingeniously avoid the above limitations, we dynamically deploy specialized high-performance networks to edge clients based on their local resource overhead.  Clients with the resource-aware model deployment can efficiently utilize their local resources and enable better downstream tasks.
% \subsection{Ablation Study}
% \subsection{Effect of knowledge network size}
% \subsection{Effect of Network capacity}
% \subsection{Effect of cloud algorithm}


==> cvpr2023/Figures/f_avg_100_01_cifar100.tex <==
\begin{figure*}[t]
 \begin{center}

% Resnet50 (res18, res32) (1-2), Mobilenetv3 (res18, res32) (3-4)
\centerline{\includegraphics[width=\linewidth]
{cvpr2023/Figures/avg_avgtl_100_01_cifar100_combined.pdf}
% {cvpr2023/Figures/vanilla-1.pdf}
}
\centerline{\includegraphics[width=1\linewidth]{cvpr2023/Figures/ensemble_avgtl_30_04_cifar10_combined.pdf}}
% \centerline{\includegraphics[width=1\linewidth]{cvpr2023/Figures/tiny_100_04_ce5_cs15_fused.pdf}}
%avg_100_01_cifar100 % Resnet50(1-2) MobileNetV3(3-4)
% \centerline{\includegraphics[width=\linewidth]{Figures/avg_100_01_cifar100.pdf}}
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_30_04_ce5_cs15.pdf}}
% mobilenetv3
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_50_07_ce5_cs15_mobile.pdf}}
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_100_04_ce5_cs15_fused.pdf}}
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_30_04_ce5_cs15.pdf}}
% mobilenetv3
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_50_07_ce5_cs15_mobile.pdf}}
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_100_04_ce5_cs15_fused.pdf}}
\caption{Supplementary results: comparison of \proj with SoTAs (numbers in parenthesis represents the communication cost per round).}
\vspace{-1em}
\label{fig:learn_efficiency}
\end{center}
 \end{figure*}

==> cvpr2023/Figures/f_avgtl_30_04_cifar10.tex <==
\begin{figure*}[t]
 \begin{center}
% MobileNetV3
\centerline{\includegraphics[width=\linewidth]{Figures/avgtl_30_04_mobile_cifar10.pdf}}
% Resnet50
% \centerline{\includegraphics[width=\linewidth]{Figures/avgtl_50_07_cifar10.pdf}}
% Resnet50(1,2) MobileNetV3(3,4)
% \centerline{\includegraphics[width=\linewidth]{Figures/avgtl_100_01_cifar100_fused.pdf}}
\caption{Comparison of \proj with SoTAs: the top-1 average test accuracy vs. communication rounds between \proj and other methods on Cifar-10/100 dataset. \proj uses averaging together with transfer learning. Bandwidth per round is included with each method.}
\vspace{-1em}
\label{fig:avgtl_30_04}
\end{center}
 \end{figure*}

==> cvpr2023/Figures/f_client_overhead.tex <==
\begin{figure}
 \begin{center}
 \vspace{-6 px}

\centerline{\includegraphics[width=1.0\columnwidth]{cvpr2023/Figures/client_overhead.pdf}}

\caption{Client overhead in \proj.}
\vspace{-6 px}
\label{fig:client_overhead}
\end{center}
 \end{figure}

==> cvpr2023/Figures/f_comm_cost.tex <==
% \begin{figure}
%  \begin{center}
% \begin{subfigure}{.48\columnwidth}
% \centerline{\includegraphics[width=\columnwidth]{cvpr2023/Figures/comm_target.pdf}}
% \end{subfigure}
% \begin{subfigure}{.48\columnwidth}
% \centerline{\includegraphics[width=\columnwidth]{cvpr2023/Figures/comm_target-v2.pdf}}
% \end{subfigure}
% \caption{Communication cost to achieve target accuracy.}
% \vspace{-1em}
% \label{fig:comm_target}
% \end{center}
%  \end{figure}
 
 
\begin{figure}[]
\begin{center}
 \vspace{-6 px}

\centerline{\includegraphics[width=.5\columnwidth]{cvpr2023/Figures/test.pdf}}
% \vspace{-.5 cm}

\caption{Communication cost to achieve target accuracy.}
% \vspace{-1.3 cm}
\label{fig:comm_target}
\end{center}
 \end{figure}

==> cvpr2023/Figures/f_ensemble_tiny_cifar10.tex <==
\begin{figure*}[t]
 \begin{center}

% Resnet50 for ensemble (b), MobileNetv3 for avgtl (c)
\centerline{\includegraphics[width=1\linewidth]{cvpr2023/Figures/ensemble_avgtl_30_04_cifar10_combined.pdf}}

% resnet50
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_30_04_ce5_cs15.pdf}}
% mobilenetv3
% \centerline{\includegraphics[width=1\linewidth]{Figures/tiny_50_07_ce5_cs15_mobile.pdf}}
\centerline{\includegraphics[width=1\linewidth]{Figures/tiny_100_04_ce5_cs15_fused.pdf}}
\caption{Comparison of \proj with SoTAs: the top-1 average test accuracy vs. communication rounds between \proj and other methods on Cifar-10 dataset. \proj uses ensemble with the presence of public data on server (b) and averaging together with transfer learning (c). Bandwidth per round is included with each method.}
\vspace{-1em}
\label{fig:ensemble_cifar10}
\end{center}
 \end{figure*}

==> cvpr2023/Figures/f_femnist.tex <==
\begin{figure}[]
 \begin{center}

\centerline{\includegraphics[width=.7\linewidth]{cvpr2023/Figures/femnist_3k_01.pdf}}
\caption{Comparison of \proj with FedAvg on FEMNIST.}
\vspace{-6px}
\label{fig:femnist}
\end{center}
 \end{figure}

==> cvpr2023/Tables/apdx/t_learning_efficient_cifar100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison on Learning Efficiency}
\label{tab:apdx_le_cifar100}
\resizebox{.5\linewidth}{!}
{%
\begin{tabular}{cccccccc}
\hline
Method                   & Dataset                   & Model       & Capacity & Clients & Participation & Round Cost & Accuracy \\ \hline
\multirow{3}{*}{FedAvg}  & \multirow{3}{*}{CIFAR100} & ResNet      & 76MFLOPs & 100     & 10\%          & 0.85GB     & 41\%     \\
                         &                           & MobileNetV2 & 15MFLOPs & 100     & 10\%          & xxGB       & 29\%     \\
                         &                           & MobileNetV3 & 9MFLOPs  & 100     & 10\%          & xxGB       & 27\%     \\ \hline
\multirow{3}{*}{FedNova} & \multirow{3}{*}{CIAFR100} & ResNet      & 76MFLOPs & 100     & 10\%          & 1.70GB     & 44\%     \\
                         &                           & MobileNetV2 & 15MFLOPs & 100     & 10\%          & xxGB       & 29\%     \\
                         &                           & MobileNetV3 & 9MFLOPs  & 100     & 10\%          & xxGB       & 29\%     \\ \hline
\multirow{3}{*}{FedProx} & \multirow{3}{*}{CIFAR100} & ResNet      & 76MFLOPs & 100     & 10\%          & 0.85GB     & 38\%     \\
                         &                           & MobileNetV2 & 15MFLOPs & 100     & 10\%          & xxGB       & 27\%     \\
                         &                           & MobileNetV3 & 9MFLOPs  & 100     & 10\%          & xxGB       & 27\%     \\ \hline
\multirow{3}{*}{RaFL}    & \multirow{3}{*}{CIFAR100} & ResNet      & 74MFLOPs & 100     & 10\%          & 0.57GB     & 64\%     \\
                         &                           & MobileNetV2 & 15MFLOPs & 100     & 10\%          & xxGB       & 49\%     \\
                         &                           & MobileNetV3 & 9MFLOPs  & 100     & 10\%          & xxGB       & xx\%     \\ \hline
\end{tabular}%
}
\end{table}

==> cvpr2023/Tables/t_learning_efficiency.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Learning efficiency: 100 clients with 10 \% random participation on CIFAR-100}
\label{tab:le}
\begin{sc}

\resizebox{.5\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Method                   & Model       & Capacity & Round Cost & Accuracy \\ \hline
\multirow{3}{*}{FedAvg}  & ResNet      & 76MFLOPs & 0.85GB     & 41\%     \\
                         & MobileNetV2 & 15MFLOPs & xxGB       & 29\%     \\
                         & MobileNetV3 & 9MFLOPs  & xxGB       & 27\%     \\ \hline
\multirow{3}{*}{FedNova} & ResNet      & 76MFLOPs & 1.70GB     & 44\%     \\
                         & MobileNetV2 & 15MFLOPs & xxGB       & 29\%     \\
                         & MobileNetV3 & 9MFLOPs  & xxGB       & 29\%     \\ \hline
\multirow{3}{*}{FedProx} & ResNet      & 76MFLOPs & 0.85GB     & 38\%     \\
                         & MobileNetV2 & 15MFLOPs & xxGB       & 27\%     \\
                         & MobileNetV3 & 9MFLOPs  & xxGB       & 27\%     \\ \hline
\multirow{3}{*}{RaFL}    & ResNet      & 74MFLOPs & 0.57GB     & 64\%     \\
                         & MobileNetV2 & 15MFLOPs & xxGB       & 49\%     \\
                         & MobileNetV3 & 9MFLOPs  & xxGB       & xx\%     \\ \hline
\end{tabular}%
}
\end{sc}
\end{table}

==> cvpr2023/Tables/t_resource_aware_append.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{RaFL under different system-heterogeneous resource constraints.}
\label{tab:resource_aware_ad}
\resizebox{.7\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ Arc.\end{tabular}} &
  \textbf{Dataset} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Avg. Resource\\ Constraints\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ Model Capacity\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Resource\\ Utilization\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Converged\\ Rounds\end{tabular}} &
  \textbf{Accuracy} \\ \hline
ResNet50 &
  CIFAR100 &
  \begin{tabular}[c]{@{}c@{}}48.01 MFLOPs\\ 79.70 MFLOPs\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}47.52 MFLOPs\\ 74.35 MFLOPs\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}99\%\\ 93\%\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}400\\ 500\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}65\%\\ 62\%\end{tabular} \\ \hline
MobileNetV3 &
  CIFAR100 &
  \begin{tabular}[c]{@{}c@{}}13.57 MFLOPs\\ 15.49 MFLOPs\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}13.07 MFLOPs\\ 13.96 MFLOPs\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}96\%\\ 90\%\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}500\\ 500\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}56\%\\ 55\%\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}

==> cvpr2023/Tables/t_resource_consumption.tex <==
\begin{table}[]
\caption{Resource Consumption for single client with different methods in Federated Learning setting. All values are in MFLOPs.}
\label{tab:resource_consumption}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
\textbf{Method} &
  \textbf{Model} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Flops\\
  range\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ model Flops\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Smallest\\ model Flops\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}c@{}}FedAvg\\ FedNova\\ FedProx\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}VGG11\\ VGG16\\ ResNet20\\ ResNet32\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}552\\ 878\\ 76\\ 152\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}552\\ 878\\ 76\\ 152\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}552\\ 878\\ 76\\ 152\end{tabular} \\ \hline
RaFL &
  \begin{tabular}[c]{@{}c@{}}ResNet50\\ MobileNetV3\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}20 - 100\\ 10 - 20\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}47\\ 13\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}28\\ 10\end{tabular} \\ \hline
\end{tabular}
}
\end{table}

==> cvpr2023/Tables/t_target_acc_cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Comparison of communication cost with SoTAs to achieve 80\% accuracy.}
\label{tab:com_cost}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ (FLOPs)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Target\\ Accuracy\end{tabular}}} & \multirow{2}{*}{\textbf{Clients}} & \multirow{2}{*}{\textbf{Communication Rounds}} & \multicolumn{4}{c}{\textbf{Communication Cost}}                                     \\
                                 &                                 &                                                                                     &                                   &                                                & \textbf{Round/Client} & \textbf{Total} & \textbf{$\Delta$ Cost} & \textbf{Speed Up} \\ \hline
\multirow{3}{*}{FedAvg~\cite{mcmahan2017fedavg}}          & ResNet (40M)                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 203                                            & 2.1MB                 & 4.16GB         & 0GB                    & (1 $\times$)      \\
                                 & ResNet (76M)                       &                                                                                     &                                   & 192                                            & 3.2MB                 & 6.00GB         & 0GB                    & (1 $\times$)      \\
                                 & Mob-V2 (15M)                          &                                                                                     &                                   & 181                                            & 42MB                  & 74.24GB        & 0GB                    & (1 $\times$)      \\ \hline
\multirow{3}{*}{FedNova~\cite{wang2020fednova}}         & ResNet (40M)                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 198                                            & 4.2MB                 & 8.12GB         & +3.96GB                & (0.51 $\times$)   \\
                                 & ResNet (76M)                       &                                                                                     &                                   & 197                                            & 6.4MB                 & 12.31GB        & +6.31GB                & (0.48 $\times$)   \\
                                 & Mob-V2 (15M)                          &                                                                                     &                                   & 159                                            & 84MB                  & 130.43GB       & +56.19                 & (0.57 $\times$)   \\ \hline
\multirow{3}{*}{FedProx~\cite{li2020fedprox}}         & ResNet (40M)                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 288                                            & 2.1MB                 & 5.91GB         & +1.75GB                & (0.70 $\times$)   \\
                                 & ResNet (76M)                       &                                                                                     &                                   & 400                                            & 3.2MB                 & 12.80GB        & +6.80GB                & (0.47 $\times$)   \\
                                 & Mob-V2 (15M)                          &                                                                                     &                                   & 296                                            & 42MB                  & 121.41GB       & +47.17GB               & (0.61 $\times$)   \\ \hline
\multirow{3}{*}{SCAFFOLD~\cite{karimireddy2020scaffold}}        & ResNet (40M)                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 49                                             & 4.3MB                 & 2.10GB         & -2.06GB                & (1.98 $\times$)   \\
                                 & ResNet (76M)                       &                                                                                     &                                   & 55                                             & 6.5MB                 & 3.60GB         & -2.40GB                & (1.67 $\times$)   \\
                                 & Mob-V2 (15M)                          &                                                                                     &                                   & 54                                             & 84MB                  & 45.00GB        & -29.24GB               & (1.65 $\times$)   \\ \hline
\multirow{3}{*}{SPATL (Ours)}    & ResNet (40M)                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 52                                             & 2.1MB                 & 1.10GB         & -3.06GB                & (3.78 $\times$)   \\
                                 & ResNet (76M)                       &                                                                                     &                                   & 50                                             & 3.6MB                 & 1.80GB         & -4.20GB                & (3.33 $\times$)   \\
                                 & Mob-V2 (15M)                          &                                                                                     &                                   & 46                                             & 61.3MB                & 28.00GB        & -46.24GB               & (2.65 $\times$)   \\ \hline
\end{tabular}%
}
\end{table*}

==> cvpr2023/algo/a01_local_update.tex <==


\begin{algorithm}[tb]

\caption{Local updates knowledge fusion with DML}
\label{alg:local}
\textbf{ClientUpdate}
\begin{algorithmic}[1] %[1] enables line numbers
\STATE $\theta_{l} \leftarrow$ local specialized model
\STATE $\theta_{l}^k \leftarrow$ knowledge network 
\STATE $\mathcal{B} \leftarrow$ split local dataset into batches 
\FOR{epoch $=1,2,\ldots, E$}
\FOR{batch $b\in \mathcal{B}$}
\STATE Perform Deep Mutual Learning:
% \STATE $\theta_{l} \leftarrow \theta_{l} - \eta \triangledown(\mathcal{L}_{\theta_l}(\theta_{l};b) + D_{KL}(\theta_{l}^k||\theta_{l})) $ 
\STATE $\theta_{l} \leftarrow \theta_{l} - \eta \triangledown(\mathcal{L}_{\theta_l}) $ 
\STATE $\theta_{l}^k \leftarrow \theta_{l}^k - \eta \triangledown(\mathcal{L}_{\theta_l}^k) $ 

% \STATE $\theta_{l}^k \leftarrow \theta_{l}^k - \eta \triangledown(\mathcal{L}(\theta_{l}^k;b) + D_{KL}(\theta_{l}||\theta_{l}^k)) $ 
\ENDFOR
\ENDFOR
\STATE \textbf{Deploy} $\theta_{l}$ locally
\STATE \textbf{Communicate} $\theta_{l}^k$
\end{algorithmic}

\end{algorithm}



==> cvpr2023/algo/a02_server.tex <==
\begin{algorithm}[tb]
\caption{Cloud ensemble knowledge distillation}
\label{alg:server}
\textbf{Server executes:}
\begin{algorithmic}[1] %[1] enables line numbers

\FOR{each round $t =1, 2,\ldots, T$}
\STATE $S \leftarrow$ subset of selected clients $\in N$
\FOR{each client $l \in S$ in parallel}
\STATE \textbf{Communicate with client $l$}.
\STATE  $\theta_{l}^k \leftarrow$ ClientUpdate on $l^{th}$ client
\ENDFOR
\STATE $\theta^k \leftarrow \frac{n_l}{N_S} \sum_{l \in S} \theta_l^k$
\IF {public data $P$ presents}
\STATE $\theta_{ens} = $ ensemble$(\{\theta_{l}^k\}_{l\in S})$
\STATE  $\theta^k \leftarrow \theta^k - \eta \triangledown(\mathcal{L}_d(\theta_{ens},\theta^k; P)) $ 
\ENDIF
\ENDFOR

\end{algorithmic}
\end{algorithm}

==> cvpr2023/figtex/fl_aggregation.tex <==
\begin{figure}
\begin{center}
 \vspace{-6 px}

\centerline{\includegraphics[width=.5\columnwidth]{cvpr2023/Figures/FL_aggregation.png}}
\vspace{-.5 cm}

\caption{Traditional FL model aggregation: The server aggregates locally trained models using a weighted sum of local model weights or gradients (Equation~\ref{eq:gradient_ag} and \ref{eq:weight_ag}), necessitating identical model architectures to prevent matrix dimension mismatches. Our framework overcomes these limitations making it possible to use different model architectures.}
\vspace{-.7 cm}
\label{fig:fl_aggregation}
\end{center}
 \end{figure}

==> cvpr2023/figtex/network_updates.tex <==
\begin{figure}%
    \centering
    \subfloat[\centering Server ensembles students for KD.]{{\includegraphics[width=0.4\linewidth]{Figures/FL_KD_global.png} }}%
    \qquad
    \subfloat[\centering Client's use DML to train their student.]{{\includegraphics[width=0.4\linewidth]{Figures/FL_KD_local.png} }}%
    \caption{The server ensembles uploaded students to generate soft labels for a public unlabeled dataset.
The soft-labels and unlabeled data are then used to train the global student before it gets downloaded.}%
    \label{fig:example}%
\end{figure}

==> cvpr2023/figtex/resource_heto/various_resource.tex <==
\begin{figure*}[]
 \begin{center}
 % \vspace{-10 px}

\centerline{
\includegraphics[width=.5\columnwidth]{cvpr2023/Figures/resource_heto.pdf}
}
\vspace{-.45 cm}
\caption{\proj under resource heterogeneous setting.}
\vspace{-.5 cm}
\label{fig:resource_heto}
\end{center}
 \end{figure*}
